Finite-dimensional Quantum Observables are the Special Symmetric Dagger-Frobenius Algebras of CP Maps

We use purity, a principle borrowed from the foundations of quantum information, to show that all special symmetric dagger-Frobenius algebras in CPM(fHilb) are canonical, i.e. that they arise by doubling of special symmetric dagger-Frobenius algebras in fHilb. In particular, this applies to all classical structures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{432}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.21}{10.4204/EPTCS.394.21}}
\pdfoutput=1

